Human Motion Detection Using Sharpened Dimensionality Reduction and Clustering

Sharpened dimensionality reduction (SDR), which belongs to the class of multidimensional projection techniques, has recently been introduced to tackle the challenges in the exploratory and visual analysis of high-dimensional data. SDR has been applied to various real-world datasets, such as human activity sensory data and astronomical datasets. However, manually labeling the samples from the generated projection are expensive. To address this problem, we propose here to use clustering methods such as k-means, Hierarchical Clustering, Density-Based Spatial Clustering of Applications with Noise (DBSCAN), and Spectral Clustering to easily label the 2D projections of high-dimensional data. We test our pipeline of SDR and the clustering methods on a range of synthetic and real-world datasets, including two different public human activity datasets extracted from smartphone accelerometer or gyroscope recordings of various movements. We apply clustering to assess the visual cluster separation of SDR, both qualitatively and quantitatively. We conclude that clustering SDR results yields better labeling results than clustering plain DR, and that k-means is the recommended clustering method for SDR in terms of clustering accuracy, ease-of-use, and computational scalability.

==> arxiv - icbhi paper/tables/accuracy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
\caption{Average accuracy for \textit{k}-means, HC (complete and ward), DBSCAN, and SC on LMDS- and SLMDS-processed real-world data.}
\label{tab:accuracy}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
                          &       & $k$-means & \begin{tabular}[c]{@{}c@{}}HC\\ (complete)\end{tabular} & \begin{tabular}[c]{@{}c@{}}HC\\ (ward)\end{tabular} & DBSCAN & SC \\ \hline
% \multirow{2}{*}{HAD}      & LMDS  & 0.7089    & 0.5415                                                            & 0.6571                                                        & 0.4723 & 0.6591   \\
%                           & SLMDS & 0.8137    & 0.8128                                                            & 0.8039                                                        & 0.6624 & 0.8488   \\ \hline
% \multirow{2}{*}{HAR}      & LMDS  & 0.5368    & 0.4822                                                            & 0.5639                                                        & 0.3641 & 0.5141   \\
%                           & SLMDS & 0.6249    & 0.6005                                                            & 0.634                                                         & 0.5459 & 0.6305   \\ \hline
\multirow{2}{*}{HAD*}     & LMDS  & 0.8149    & 0.5745                                                            & 0.7796                                                        & 0.5730  & 0.8278   \\
                          & SLMDS & 0.9713    & 0.9388                                                            & 0.9637                                                        & 0.7063 & 0.7583   \\ \hline
\multirow{2}{*}{HAR*}     & LMDS  & 0.9829    & 0.4971                                                            & 0.9845                                                        & 0.8107 & 0.9763   \\
                          & SLMDS & 0.9961    & 0.9961                                                            & 0.9961                                                        & 0.9942 & 0.9961   \\ \hline
\multirow{2}{*}{WiFi}     & LMDS  & 0.9160     & 0.8915                                                            & 0.9040                                                         & 0.2714 & 0.9055   \\
                          & SLMDS & 0.9395    & 0.9395                                                            & 0.9395                                                        & 0.9273 & 0.7709   \\ \hline
\multirow{2}{*}{Banknote} & LMDS  & 0.5758    & 0.6793                                                            & 0.5328                                                        & 0.4932 & 0.5364   \\
                          & SLMDS & 0.6844    & 0.7828                                                            & 0.6844                                                        & 0.3134 & 0.5871   \\ \hline
\end{tabular}
}
\end{table}

==> arxiv - icbhi paper/tables/accuracy_wo_lmds.tex <==
\begin{table*}[ht]
\centering
  \footnotesize \onehalfspacing
  \caption{Average accuracy of \textit{k}-means, hierarchical clustering (complete and ward linkage), DBSCAN, and spectral clustering on SLMDS-processed data}
  \begin{tabular}{cccccc}
     \hline
     \normalfont Data & \textit{k}-means & \begin{tabular}{@{}c@{}}Hierarchical \\ (complete)\end{tabular} & \begin{tabular}{@{}c@{}}Hierarchical \\ (ward)\end{tabular} & DBSCAN & Spectral\\
     \hline
     HAD & 0.8137 & 0.8128 & 0.8039 & 0.6624 & 0.8488\\
     HAR & 0.6249 & 0.6005 & 0.6340 & 0.5459 & 0.6301\\
     HAD$^*$ & 0.9713 & 0.9388 & 0.9637 & 0.7063 & 0.7583\\
     HAR$^*$ & 0.9961 & 0.9961 & 0.9961 & 0.9942 & 0.9961\\
     Wifi & 0.9395 & 0.9395 & 0.9395 & 0.9273 & 0.8477 \\
     Banknote & 0.6844 & 0.7828 & 0.6844 & 0.3676 & 0.5649 \\
     \hline
  \end{tabular}
  \label{tab:accuracy}
\end{table*}

==> arxiv - icbhi paper/tables/nmi.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
\caption{Average NMI for \textit{k}-means, HC (complete and ward), DBSCAN, and SC on LMDS- and SLMDS-processed real-world data.}
\label{tab:nmi}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
                          &       & $k$-means & \begin{tabular}[c]{@{}c@{}}HC\\ (complete)\end{tabular} & \begin{tabular}[c]{@{}c@{}}HC\\ (ward)\end{tabular} & DBSCAN & SC \\ \hline
%\multirow{2}{*}{HAD}      & LMDS  & 0.6445    & 0.5656                                                            & 0.6689                                                        & 0.5546 & 0.6534   \\
%                          & SLMDS & 0.8161    & 0.7705                                                            & 0.8059                                                        & 0.7189 & 0.8149   \\ \hline
%\multirow{2}{*}{HAR}      & LMDS  & 0.6006    & 0.6135                                                            & 0.6075                                                        & 0.6119 & 0.59     \\
%                          & SLMDS & 0.6451    & 0.6754                                                            & 0.6722                                                        & 0.7433 & 0.616    \\ \hline
\multirow{2}{*}{HAD*}     & LMDS  & 0.7101    & 0.5930                                                             & 0.7471                                                        & 0.5880  & 0.7077   \\
                          & SLMDS & 0.9090     & 0.8441                                                            & 0.8969                                                        & 0.7656 & 0.8106   \\ \hline
\multirow{2}{*}{HAR*}     & LMDS  & 0.9306    & 0.2566                                                            & 0.9313                                                        & 0.7975 & 0.9110    \\
                          & SLMDS & 0.9767    & 0.9767                                                            & 0.9767                                                        & 0.9705 & 0.9767   \\ \hline
\multirow{2}{*}{WiFi}     & LMDS  & 0.7887    & 0.7386                                                            & 0.7611                                                        & 0.0549 & 0.7759   \\
                          & SLMDS & 0.8686    & 0.8686                                                            & 0.8686                                                        & 0.8536 & 0.7682   \\ \hline
\multirow{2}{*}{Banknote} & LMDS  & 0.0184    & 0.2068                                                            & 0.0045                                                        & 0.2106 & 0.0123   \\
                          & SLMDS & 0.2094    & 0.4044                                                            & 0.2094                                                        & 0.5311 & 0.0718   \\ \hline
\end{tabular}
}
\end{table}

==> arxiv - icbhi paper/tables/nmi_wo_lmds.tex <==
\begin{table*}[ht]
\centering
  \footnotesize \onehalfspacing
  \caption{Average NMI of \textit{k}-means, hierarchical clustering (complete and ward linkage), DBSCAN, and spectral clustering on SLMDS-processed data}
  \begin{tabular}{cccccc}
     \hline
     \normalfont Data & \textit{k}-means & \begin{tabular}{@{}c@{}}Hierarchical \\ (complete)\end{tabular} & \begin{tabular}{@{}c@{}}Hierarchical \\ (ward)\end{tabular} & DBSCAN & Spectral\\
     \hline
     HAD & 0.8161 & 0.7705 & 0.8059 & 0.7189 & 0.8149\\
     HAR & 0.6451 & 0.6754 & 0.6722 & 0.7433 & 0.6159\\
     HAD$^*$ & 0.9090 & 0.8441 & 0.8969 & 0.7656 & 0.8106\\
     HAR$^*$ & 0.9767 & 0.9767 & 0.9767 & 0.9705 & 0.9767 \\
     Wifi & 0.8686 & 0.8686 & 0.8686 & 0.8536 & 0.8063 \\
     Banknote & 0.2684 & 0.4044 & 0.2094 & 0.5311 & 0.0807 \\
     \hline
  \end{tabular}
  \label{tab:NMI}
\end{table*}

==> arxiv - icbhi paper/tables/only_HAD_HAR_acc_pur_nmi.tex <==
\begin{table*}[ht]
\centering
  \footnotesize \onehalfspacing
  \caption{Average accuracy, purity, NMI scores for \textit{k}-means, hierarchical clustering (complete and ward linkage), DBSCAN, and spectral clustering on SLMDS-processed HAD and HAR data sets}
  \begin{tabular}{ccccccc}
     \hline
     \normalfont Measurement & Data & \textit{k}-means & \begin{tabular}{@{}c@{}}Hierarchical \\ (complete)\end{tabular} & \begin{tabular}{@{}c@{}}Hierarchical \\ (ward)\end{tabular} & DBSCAN & Spectral\\
     \hline
     Accuracy & HAD & 0.8137 & 0.8128 & 0.8039 & 0.6624 & 0.8488\\
      & HAR & 0.6249 & 0.6005 & 0.6340 & 0.5459 & 0.6301\\
     Purity & HAD & 0.8704 & 0.8396 & 0.8558 & 0.7205 & 0.8577 \\
      & HAR & 0.6384 & 0.6079 & 0.6413 & 0.5468 & 0.6339\\
     NMI & HAD & 0.8161 & 0.7705 & 0.8059 & 0.7189 & 0.8149\\
      & HAR & 0.6451 & 0.6754 & 0.6722 & 0.7433 & 0.6159\\
     \hline
  \end{tabular}
  \label{tab:pureHAD_HAR_measurements}
\end{table*}

==> arxiv - icbhi paper/tables/purity.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
\caption{Average purity for \textit{k}-means, HC (complete and ward), DBSCAN, and SC on LMDS- and SLMDS-processed real-world data.}
\label{tab:purity}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccc}
\hline
                          &       & $k$-means & \begin{tabular}[c]{@{}c@{}}HC\\ (complete)\end{tabular} & \begin{tabular}[c]{@{}c@{}}HC\\ (ward)\end{tabular} & DBSCAN & SC \\ \hline
%\multirow{2}{*}{HAD}      & LMDS  & 0.7156    & 0.5627                                                            & 0.6715                                                        & 0.4762 & 0.7256   \\
%                          & SLMDS & 0.8704    & 0.8396                                                            & 0.8558                                                        & 0.7205 & 0.8577   \\ \hline
%\multirow{2}{*}{HAR}      & LMDS  & 0.6225    & 0.5828                                                            & 0.6423                                                        & 0.3651 & 0.6054   \\
%                          & SLMDS & 0.6384    & 0.6079                                                            & 0.6413                                                        & 0.5468 & 0.6342   \\ \hline
\multirow{2}{*}{HAD*}     & LMDS  & 0.8149    & 0.6190                                                             & 0.7796                                                        & 0.5785 & 0.8278   \\
                          & SLMDS & 0.9713    & 0.9388                                                            & 0.9637                                                        & 0.7646 & 0.7672   \\ \hline
\multirow{2}{*}{HAR*}     & LMDS  & 0.9829    & 0.5257                                                            & 0.9845                                                        & 0.8139 & 0.9763   \\
                          & SLMDS & 0.9961    & 0.9961                                                            & 0.9961                                                        & 0.9959 & 0.9961   \\ \hline
\multirow{2}{*}{WiFi}     & LMDS  & 0.9160     & 0.8915                                                            & 0.9040                                                         & 0.2781 & 0.9055   \\
                          & SLMDS & 0.9395    & 0.9395                                                            & 0.9395                                                        & 0.9373 & 0.7825   \\ \hline
\multirow{2}{*}{Banknote} & LMDS  & 0.5758    & 0.6793                                                            & 0.5554                                                        & 0.7252 & 0.5554   \\
                          & SLMDS & 0.6844    & 0.7828                                                            & 0.6844                                                        & 0.9785 & 0.5906   \\ \hline
\end{tabular}
}
\end{table}

==> arxiv - icbhi paper/tables/purity_wo_lmds.tex <==
\begin{table*}[ht]
\centering
  \footnotesize \onehalfspacing
  \caption{Average purity of \textit{k}-means, hierarchical clustering (complete and ward linkage), DBSCAN, and spectral clustering on SLMDS-processed data}
  \begin{tabular}{cccccc}
     \hline
     \normalfont Data & \textit{k}-means & \begin{tabular}{@{}c@{}}Hierarchical \\ (complete)\end{tabular} & \begin{tabular}{@{}c@{}}Hierarchical \\ (ward)\end{tabular} & DBSCAN & Spectral\\
     \hline
     HAD & 0.8704 & 0.8396 & 0.8558 & 0.7205 & 0.8577 \\
     HAR & 0.6384 & 0.6079 & 0.6413 & 0.5468 & 0.6339\\
     HAD$^*$ & 0.9713 & 0.9388 & 0.9637 & 0.7646 & 0.7672\\
     HAR$^*$ & 0.9961 & 0.9961 & 0.9961 & 0.9959 & 0.9961 \\
     Wifi & 0.9395 & 0.9395 & 0.9395 & 0.9373 & 0.8535 \\
     Banknote & 0.7344 & 0.7828 & 0.6844 & 0.9785 & 0.5832 \\
     \hline
  \end{tabular}
  \label{tab:purity}
\end{table*}

==> tables/accuracy_wo_lmds.tex <==
\begin{table*}[ht]
\centering
  \footnotesize \onehalfspacing
  \caption{Average accuracy of \textit{k}-means, hierarchical clustering (complete and ward linkage), DBSCAN, and spectral clustering on SLMDS-processed data}
  \begin{tabular}{cccccc}
     \hline
     \normalfont Data & \textit{k}-means & \begin{tabular}{@{}c@{}}Hierarchical \\ (complete)\end{tabular} & \begin{tabular}{@{}c@{}}Hierarchical \\ (ward)\end{tabular} & DBSCAN & Spectral\\
     \hline
     HAD & 0.8137 & 0.8128 & 0.8039 & 0.6624 & 0.8488\\
     HAR & 0.6249 & 0.6005 & 0.6340 & 0.5459 & 0.6301\\
     HAD$^*$ & 0.9713 & 0.9388 & 0.9637 & 0.7063 & 0.7583\\
     HAR$^*$ & 0.9961 & 0.9961 & 0.9961 & 0.9942 & 0.9961\\
     Wifi & 0.9395 & 0.9395 & 0.9395 & 0.9273 & 0.8477 \\
     Banknote & 0.6844 & 0.7828 & 0.6844 & 0.3676 & 0.5649 \\
     \hline
  \end{tabular}
  \label{tab:accuracy}
\end{table*}

==> tables/nmi_wo_lmds.tex <==
\begin{table*}[ht]
\centering
  \footnotesize \onehalfspacing
  \caption{Average NMI of \textit{k}-means, hierarchical clustering (complete and ward linkage), DBSCAN, and spectral clustering on SLMDS-processed data}
  \begin{tabular}{cccccc}
     \hline
     \normalfont Data & \textit{k}-means & \begin{tabular}{@{}c@{}}Hierarchical \\ (complete)\end{tabular} & \begin{tabular}{@{}c@{}}Hierarchical \\ (ward)\end{tabular} & DBSCAN & Spectral\\
     \hline
     HAD & 0.8161 & 0.7705 & 0.8059 & 0.7189 & 0.8149\\
     HAR & 0.6451 & 0.6754 & 0.6722 & 0.7433 & 0.6159\\
     HAD$^*$ & 0.9090 & 0.8441 & 0.8969 & 0.7656 & 0.8106\\
     HAR$^*$ & 0.9767 & 0.9767 & 0.9767 & 0.9705 & 0.9767 \\
     Wifi & 0.8686 & 0.8686 & 0.8686 & 0.8536 & 0.8063 \\
     Banknote & 0.2684 & 0.4044 & 0.2094 & 0.5311 & 0.0807 \\
     \hline
  \end{tabular}
  \label{tab:NMI}
\end{table*}

==> tables/only_HAD_HAR_acc_pur_nmi.tex <==
\begin{table*}[ht]
\centering
  \footnotesize \onehalfspacing
  \caption{Average accuracy, purity, NMI scores for \textit{k}-means, hierarchical clustering (complete and ward linkage), DBSCAN, and spectral clustering on SLMDS-processed HAD and HAR data sets}
  \begin{tabular}{ccccccc}
     \hline
     \normalfont Measurement & Data & \textit{k}-means & \begin{tabular}{@{}c@{}}Hierarchical \\ (complete)\end{tabular} & \begin{tabular}{@{}c@{}}Hierarchical \\ (ward)\end{tabular} & DBSCAN & Spectral\\
     \hline
     Accuracy & HAD & 0.8137 & 0.8128 & 0.8039 & 0.6624 & 0.8488\\
      & HAR & 0.6249 & 0.6005 & 0.6340 & 0.5459 & 0.6301\\
     Purity & HAD & 0.8704 & 0.8396 & 0.8558 & 0.7205 & 0.8577 \\
      & HAR & 0.6384 & 0.6079 & 0.6413 & 0.5468 & 0.6339\\
     NMI & HAD & 0.8161 & 0.7705 & 0.8059 & 0.7189 & 0.8149\\
      & HAR & 0.6451 & 0.6754 & 0.6722 & 0.7433 & 0.6159\\
     \hline
  \end{tabular}
  \label{tab:pureHAD_HAR_measurements}
\end{table*}

==> tables/purity_wo_lmds.tex <==
\begin{table*}[ht]
\centering
  \footnotesize \onehalfspacing
  \caption{Average purity of \textit{k}-means, hierarchical clustering (complete and ward linkage), DBSCAN, and spectral clustering on SLMDS-processed data}
  \begin{tabular}{cccccc}
     \hline
     \normalfont Data & \textit{k}-means & \begin{tabular}{@{}c@{}}Hierarchical \\ (complete)\end{tabular} & \begin{tabular}{@{}c@{}}Hierarchical \\ (ward)\end{tabular} & DBSCAN & Spectral\\
     \hline
     HAD & 0.8704 & 0.8396 & 0.8558 & 0.7205 & 0.8577 \\
     HAR & 0.6384 & 0.6079 & 0.6413 & 0.5468 & 0.6339\\
     HAD$^*$ & 0.9713 & 0.9388 & 0.9637 & 0.7646 & 0.7672\\
     HAR$^*$ & 0.9961 & 0.9961 & 0.9961 & 0.9959 & 0.9961 \\
     Wifi & 0.9395 & 0.9395 & 0.9395 & 0.9373 & 0.8535 \\
     Banknote & 0.7344 & 0.7828 & 0.6844 & 0.9785 & 0.5832 \\
     \hline
  \end{tabular}
  \label{tab:purity}
\end{table*}
